Universal Domain Adaptation for Robust Handling of Distributional Shifts in NLP

When deploying machine learning systems to the wild, it is highly desirable for them to effectively leverage prior knowledge to the unfamiliar domain while also firing alarms to anomalous inputs. In order to address these requirements, Universal Domain Adaptation (UniDA) has emerged as a novel research area in computer vision, focusing on achieving both adaptation ability and robustness (i.e., the ability to detect out-of-distribution samples). While UniDA has led significant progress in computer vision, its application on language input still needs to be explored despite its feasibility. In this paper, we propose a comprehensive benchmark for natural language that offers thorough viewpoints of the model's generalizability and robustness. Our benchmark encompasses multiple datasets with varying difficulty levels and characteristics, including temporal shifts and diverse domains. On top of our testbed, we validate existing UniDA methods from computer vision and state-of-the-art domain adaptation techniques from NLP literature, yielding valuable findings: We observe that UniDA methods originally designed for image input can be effectively transferred to the natural language domain while also underscoring the effect of adaptation difficulty in determining the model's performance.

==> Assets/Figures/_NOT_USED__msp_all.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/ft_known.pdf}
        \caption{Fine-tuning}
        \label{figure:ft_known_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/dann_known.pdf}
        \caption{DANN}
        \label{figure:dann_known_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/udalm_known.pdf}
        \caption{UDALM}
        \label{figure:udalm_known_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/adspt_known.pdf}
        \caption{AdSPT}
        \label{figure:adspt_known_dist}
    \end{subfigure}
            
    \caption{
        Maximum Softmax Probability Distribution of \textit{known} samples for different CDA methods.
        As the domain discrepancy enlarges, the MSP distribution becomes more uncertain.
    }
    \label{figure:known_dist}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/ft_unknown.pdf}
        \caption{Fine-tuning}
        \label{figure:ft_unknown_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/dann_unknown.pdf}
        \caption{DANN}
        \label{figure:dann_unknown_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/udalm_unknown.pdf}
        \caption{UDALM}
        \label{figure:udalm_unknown_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp/adspt_unknown.pdf}
        \caption{AdSPT}
        \label{figure:adspt_unknown_dist}
    \end{subfigure}
            
    \caption{
        Maximum Softmax Probability Distribution of \textit{unknown} samples for different CDA methods.
        Regardless of the domain discrepancy, the \textit{unknown} samples consistently show low confidence.
    }
    \label{figure:unknown_dist}
\end{figure*}

==> Assets/Figures/_NOT_USED__msp_v2.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/udalm_2013.pdf}
        \caption{UDALM (2013)}
        \label{figure:udalm_20173msp}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/udalm_2014.pdf}
        \caption{UDALM (2014)}
        \label{figure:udalm_2014_msp}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/udalm_2015.pdf}
        \caption{UDALM (2015)}
        \label{figure:udalm_2015_msp}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/udalm_2016.pdf}
        \caption{UDALM (2016)}
        \label{figure:udalm_2016_msp}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/udalm_2017.pdf}
        \caption{UDALM (2017)}
        \label{figure:udalm_2017_msp}
    \end{subfigure}
            
    \caption{
        H-score performance with different threshold values. 
        Methods without threshold values are visualized as a horizontal line.
    }
    \label{figure:udalm_msp}
\end{figure*}

==> Assets/Figures/analysis_main.tex <==



\begin{figure*}[t]
    % \centering
    % \begin{subfigure}{0.328\textwidth}
    %     \includegraphics[width=\textwidth]{Assets/Figures/analysis/cda_known.pdf}
    %     \caption{Known accuracy of CDA methods}
    %     \label{figure:cda_known}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.328\textwidth}
    %     \includegraphics[width=\textwidth]{Assets/Figures/analysis/cda_unknown.pdf}
    %     \caption{Unknown accuracy of CDA methods}
    %     \label{figure:cda_unknown}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.328\textwidth}
    %     \includegraphics[width=\textwidth]{Assets/Figures/analysis/cda_hscore.pdf}
    %     \caption{H-score of CDA methods}
    %     \label{figure:cda_hscore}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.328\textwidth}
    %     \includegraphics[width=\textwidth]{Assets/Figures/analysis/unida_known.pdf}
    %     \caption{Known accuracy of UniDA methods}
    %     \label{figure:unida_known}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.328\textwidth}
    %     \includegraphics[width=\textwidth]{Assets/Figures/analysis/unida_unknown.pdf}
    %     \caption{Unknown accuracy of UniDA methods}
    %     \label{figure:unida_unknown}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.328\textwidth}
    %     \includegraphics[width=\textwidth]{Assets/Figures/analysis/unida_hscore.pdf}
    %     \caption{H-score of UniDA methods}
    %     \label{figure:unida_hscore}
    % \end{subfigure}

    \centering
    \begin{subfigure}{0.328\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/analysis/known.pdf}
        \caption{Known accuracy}
        \label{figure:known_analysis}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.328\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/analysis/unknown.pdf}
        \caption{Unknown accuracy}
        \label{figure:unknown_analysis}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.328\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/analysis/hscore.pdf}
        \caption{H-score}
        \label{figure:hscore_analysis}
    \end{subfigure}
    
    
            
    \caption{
        Overall tendency of AdSPT and UDALM in Huffpost dataset as the adaptation complexity increases.
        We also plot the values of PDR and DDS to visualize the correlations with the method's results.
        In the less challenging scenario, AdSPT demonstrates better performance,
        while OVANet exhibit superior performance as the the difficult level escalates.
    }
    \label{figure:analysis_main}
\end{figure*}

==> Assets/Figures/msp.tex <==

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{Assets/Figures/msp/adspt_2013.pdf}
        \caption{AdSPT (2013)}
        \label{figure:adspt_2013_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{Assets/Figures/msp/adspt_2017.pdf}
        \caption{AdSPT (2017)}
        \label{figure:adspt_2017_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{Assets/Figures/msp/udalm_2013.pdf}
        \caption{UDALM (2013)}
        \label{figure:udalm_2013_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{Assets/Figures/msp/udalm_2017.pdf}
        \caption{UDALM (2017)}
        \label{figure:udalm_2017_dist}
    \end{subfigure}
            
    \caption{
        Maximum Softmax Probability Distribution of \textit{known} samples (red) and \textit{unknown} samples (black) for AdSPT and UDALM.
        For an easy adaptation, the distributions show clear difference.
        However, for an challenging adaptation, both distributions show low confidence, making it difficult to discriminate the two distributions.
    }
    \label{figure:dist_2013_2017}
\end{figure}

==> Assets/Figures/msp_v2.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_2013.pdf}
        \caption{Huffpost (2012 $\rightarrow$ 2013)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_2014.pdf}
        \caption{Huffpost (2012 $\rightarrow$ 2014)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_2015.pdf}
        \caption{Huffpost (2012 $\rightarrow$ 2015)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_2016.pdf}
        \caption{Huffpost (2012 $\rightarrow$ 2016)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_2017.pdf}
        \caption{Huffpost (2012 $\rightarrow$ 2017)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_clinc.pdf}
        \caption{CLINC-150}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_amazon.pdf}
        \caption{Amazon}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \includegraphics[width=\textwidth]{Assets/Figures/msp_v2/fine_tuning_amazon.pdf}
        \caption{Amazon}
        \label{figure:msp_v2_amazon}
    \end{subfigure}
            
    \caption{
        MSP distributions
    }
    \label{figure:msp_v2}
\end{figure*}
